When to Trust Aggregated Gradients: Addressing Negative Client Sampling in Federated Learning

Federated Learning has become a widely-used framework which allows learning a global model on decentralized local datasets under the condition of protecting local data privacy. However, federated learning faces severe optimization difficulty when training samples are not independently and identically distributed (non-i.i.d.). In this paper, we point out that the client sampling practice plays a decisive role in the aforementioned optimization difficulty. We find that the negative client sampling will cause the merged data distribution of currently sampled clients heavily inconsistent with that of all available clients, and further make the aggregated gradient unreliable. To address this issue, we propose a novel learning rate adaptation mechanism to adaptively adjust the server learning rate for the aggregated gradient in each round, according to the consistency between the merged data distribution of currently sampled clients and that of all available clients. Specifically, we make theoretical deductions to find a meaningful and robust indicator that is positively related to the optimal server learning rate and can effectively reflect the merged data distribution of sampled clients, and we utilize it for the server learning rate adaptation. Extensive experiments on multiple image and text classification tasks validate the great effectiveness of our method.

==> tables/20_local_epochs.tex <==
\begin{table}[t!]
\caption{The results of $E=20$.}
\label{tab: main results}
\small
\vskip 0.15in
\begin{center}
 \setlength{\tabcolsep}{3.0pt}
\sisetup{detect-all,mode=text}
\begin{tabular}{lcccc}
\toprule
\multirow{2.5}{*}{\begin{tabular}[c]{@{}l@{}}Method \end{tabular}} &  \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{MNIST}  \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
&  $\alpha=0.1$   &  $\alpha=1.0$  &   $\alpha=0.1$    & $\alpha=1.0$     \\
%\midrule
%\multicolumn{5}{c}{SGD Server Optimizer}  \\ 
\midrule
FedAvg  & 48.20 {\scriptsize($\pm$ 0.86)} & 74.94  {\scriptsize($\pm$ 0.95)} & 86.13 {\scriptsize($\pm$ 0.40)}  & 94.87 {\scriptsize($\pm$ 0.28)}    \\
~~ \small{+ FedGLAD} &  \textbf{50.80} {\scriptsize($\pm$ 1.09)} &  \textbf{75.45} {\scriptsize($\pm$ 1.12)}  &   \textbf{87.47} {\scriptsize($\pm$ 0.35)}   &   \textbf{95.10} {\scriptsize($\pm$ 0.33)}    \\
%\cmidrule{2-9}
% \midrule
\midrule
%\multicolumn{5}{c}{Advanced Server Optimizer}  \\ 
%\midrule
FedAvgM &  52.26 {\scriptsize($\pm$ 1.73)} &  69.80 {\scriptsize($\pm$ 0.63)}  &  86.20 {\scriptsize($\pm$ 2.55)}  & 96.51 {\scriptsize($\pm$ 0.52)}     \\
~~ \small{+ FedGLAD} &  \textbf{55.16} {\scriptsize($\pm$ 1.76)}   &  \textbf{70.36} {\scriptsize($\pm$ 0.68)} &   \textbf{86.68} {\scriptsize($\pm$ 2.68)}   & \textbf{97.09} {\scriptsize($\pm$ 0.53)}    \\
%\cmidrule{2-9}
% \midrule
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}

==> tables/different_sampling_ratios.tex <==
\begin{table}[t]
\caption{The results of using different sampling ratios.}
\label{tab: different sampling ratios}
\vskip 0.15in
\begin{center}
 \setlength{\tabcolsep}{6.0pt}
\begin{small}
%\begin{sc}
\begin{tabular}{llccc}
\toprule
\multirow{2.5}{*}{Dataset} & \multirow{2.5}{*}{Method} & \multicolumn{3}{c}{Sampling Ratio}  \\
\cmidrule(lr){3-5}
 & & 5\% & 10\% & 20\%  \\
\midrule
\multirow{4.5}{*}{CIFAR-10} & FedAvg &  29.91 & 35.30  & 52.05 \\
& ~~ \small{+ FedGLAD} & \textbf{33.35} & \textbf{38.44} & \textbf{53.40} \\ 
\cmidrule{2-5}
 & FedAvgM & 34.72  & 48.79 & 63.56  \\
 & ~~ \small{+ FedGLAD} & \textbf{36.48} & \textbf{50.91}  & \textbf{63.84} \\
\cmidrule{1-5}
\multirow{4.5}{*}{20NewsGroups} & FedAvg & 63.09 & 72.84  & 76.31 \\
& ~~ \small{+ FedGLAD} & \textbf{63.49} & \textbf{73.14}  & \textbf{76.35} \\ 
\cmidrule{2-5}
 & FedAvgM & 61.51 & 75.44  & \textbf{80.08} \\
 & ~~ \small{+ FedGLAD} & \textbf{62.48} & \textbf{75.91}  & 79.98 \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/impact_on_scale_component.tex <==
\begin{table}[t]
\caption{The averaged ratio values between the mean and standard deviation of uploaded local gradients in different settings.}
\label{tab: impact on scale component}
\vskip 0.15in
\begin{center}
%\setlength{\tabcolsep}{4.0pt}
\begin{small}
%\begin{sc}
\begin{tabular}{lcccc}
\toprule
\multirow{2.5}{*}{Dataset} & \multirow{2.5}{*}{$\alpha$} & \multicolumn{3}{c}{Local Epochs}  \\
\cmidrule(lr){3-5}
 & & 1 & 3 & 5\\
\midrule
\multirow{2.5}{*}{CIFAR-10} & 0.1 & 0.23 & 0.29  & 0.32 \\
\cmidrule{2-5}
& 1.0 & 0.23 & 0.19 & 0.15 \\
\midrule
\multirow{2.5}{*}{20NewsGroups} & 0.1 & 0.12  &  0.15 & 0.16\\
\cmidrule{2-5}
& 1.0 & 0.08 & & 0.14 \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



==> tables/main_results.tex <==
\begin{table*}[t!]
\caption{The main results of all baselines with (+FedGLAD) or without our method in different non-i.i.d.\ degree settings}
\label{tab: main results}
\small
\vskip 0.1in
\begin{center}
 \setlength{\tabcolsep}{3.0pt}
\sisetup{detect-all,mode=text}
\resizebox{.99\textwidth}{!}
{

\begin{tabular}{lcccccccc}
\toprule
\multirow{2.5}{*}{\begin{tabular}[c]{@{}l@{}}Method \end{tabular}} &  \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{20NewsGroups} & \multicolumn{2}{c}{AGNews} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
&  $\alpha=0.1$   &  $\alpha=1.0$  &   $\alpha=0.1$    & $\alpha=1.0$    & $\alpha=0.1$  & $\alpha=1.0$   &  $\alpha=0.1$ & $\alpha=1.0$   \\
\midrule
\multicolumn{9}{c}{SGD Server Optimizer}  \\ 
\midrule
FedAvg  & 35.30 {\scriptsize($\pm$ 1.62)} &  72.09 {\scriptsize($\pm$ 1.27)} & 78.17 {\scriptsize($\pm$ 0.35)}  & 91.42 {\scriptsize($\pm$ 0.11)} & 72.84 {\scriptsize($\pm$ 0.12)}  & 76.66 {\scriptsize($\pm$ 0.36)} & 79.48 {\scriptsize($\pm$ 0.46)} & 91.27 {\scriptsize($\pm$ 0.04)}  \\
~~ \small{+ FedGLAD} &  \textbf{38.44} {\scriptsize($\pm$ 0.91)} & \textbf{72.79} {\scriptsize($\pm$ 1.13)}  &   \textbf{79.71} {\scriptsize($\pm$ 0.49)}   &   \textbf{91.63} {\scriptsize($\pm$ 0.08)} &  \textbf{73.14} {\scriptsize($\pm$ 0.08)}  &  \textbf{77.21} {\scriptsize($\pm$ 0.42)} &  \textbf{80.74} {\scriptsize($\pm$ 0.79)} &  \textbf{91.38} {\scriptsize($\pm$ 0.04)}   \\
%\cmidrule{2-9}
\midrule
FedProx &  43.48 {\scriptsize($\pm$ 0.79)} &  71.22 {\scriptsize($\pm$ 0.83)}   & 82.72 {\scriptsize($\pm$ 0.25)}  & 91.68 {\scriptsize($\pm$ 0.05)} &  72.78 {\scriptsize($\pm$ 0.20)} & 76.51 {\scriptsize($\pm$ 0.47)} & 82.61 {\scriptsize($\pm$ 0.56)}  & 91.24 {\scriptsize($\pm$ 0.09)}   \\
~~ \small{+ FedGLAD} & \textbf{44.52} {\scriptsize($\pm$ 0.72)} & \textbf{71.52} {\scriptsize($\pm$ 0.61)} & \textbf{83.54} {\scriptsize($\pm$ 0.34)}  &  \textbf{91.86} {\scriptsize($\pm$ 0.06)}  &  \textbf{73.19} {\scriptsize($\pm$ 0.08)} &  \textbf{77.13} {\scriptsize($\pm$ 0.17)} & \textbf{83.44} {\scriptsize($\pm$ 0.44)} &  \textbf{91.35} {\scriptsize($\pm$ 0.09)}  \\
\midrule
\multicolumn{9}{c}{Advanced Server Optimizer}  \\ 
\midrule
FedAvgM & 48.79 {\scriptsize($\pm$ 1.35)} & 72.63  {\scriptsize($\pm$ 0.56)}  & 81.71  {\scriptsize($\pm$ 0.99)}  & 93.37 {\scriptsize($\pm$ 0.29)}  & 75.44 {\scriptsize($\pm$ 0.10)}  & 79.51 {\scriptsize($\pm$ 0.31)} & 80.28 {\scriptsize($\pm$ 1.75)} &  90.07 {\scriptsize($\pm$ 0.27)}   \\
~~ \small{+ FedGLAD} &  \textbf{50.91} {\scriptsize($\pm$ 1.33)}   &  \textbf{73.07} {\scriptsize($\pm$ 0.33)} &   \textbf{82.11} {\scriptsize($\pm$ 0.64)}   & \textbf{93.97} {\scriptsize($\pm$ 0.26)} &  \textbf{75.91} {\scriptsize($\pm$ 0.29)}  &  \textbf{79.77} {\scriptsize($\pm$ 0.08)}&  \textbf{83.68} {\scriptsize($\pm$ 0.87)} & \textbf{90.45} {\scriptsize($\pm$ 0.42)}   \\
%\cmidrule{2-9}
\midrule
FedAdam  &  56.82 {\scriptsize($\pm$ 1.12)}  & 79.97 {\scriptsize($\pm$ 1.30)}  & 96.94 {\scriptsize($\pm$ 0.14)} & 98.42 {\scriptsize($\pm$ 0.08)} &  \textbf{76.76} {\scriptsize($\pm$ 1.17)}  & 79.96 {\scriptsize($\pm$ 0.12)} & 86.72 {\scriptsize($\pm$ 1.02)} & 91.72 {\scriptsize($\pm$ 0.12)}   \\
~~ \small{+ FedGLAD}  & \textbf{57.69} {\scriptsize($\pm$ 1.23)}   & \textbf{80.75} {\scriptsize($\pm$ 1.35)}  &  \textbf{97.11} {\scriptsize($\pm$ 0.11)}   & \textbf{98.53} {\scriptsize($\pm$ 0.04)}  & 76.59 {\scriptsize($\pm$ 0.81)} & \textbf{80.13} {\scriptsize($\pm$ 0.20)}  & \textbf{88.47} {\scriptsize($\pm$ 0.51)}  & \textbf{91.81} {\scriptsize($\pm$ 0.10)}   \\
\bottomrule
\end{tabular}
}
\end{center}
\vskip -0.15in
\end{table*}

==> tables/main_results_only_improvement.tex <==
\begin{table*}[t!]
\caption{Main improvements.}
\label{tab: main improvements}
\small
\vskip 0.15in
\begin{center}
 \setlength{\tabcolsep}{3.0pt}
\sisetup{detect-all,mode=text}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2.5}{*}{\begin{tabular}[c]{@{}l@{}}Method \end{tabular}} & \multicolumn{2}{c}{ 20NewsGroups} & \multicolumn{2}{c}{AGNews} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{MNIST} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
&  $\alpha=0.1$   &  $\alpha=1.0$  &   $\alpha=0.1$    & $\alpha=1.0$    & $\alpha=0.1$  & $\alpha=1.0$   &  $\alpha=0.1$ & $\alpha=1.0$   \\
\midrule
\texttt{FedAvg} & 72.84   & 76.66  & 79.48  & 91.27  & 48.20  & 74.94  & 86.13 & 94.87  \\
~~ \small{+ PGALRS}  &  \textbf{+0.30} {\scriptsize($\pm$ 0.10)}  &  \textbf{+0.55} {\scriptsize($\pm$ 0.35)} &  \textbf{+1.26} {\scriptsize($\pm$ 0.33)} &  \textbf{+0.11} {\scriptsize($\pm$ 0.01)}  &  \textbf{+2.60} {\scriptsize($\pm$ 1.92)} &  \textbf{+0.51} {\scriptsize($\pm$ 0.28)}  &   \textbf{+1.34} {\scriptsize($\pm$ 0.11)}   &  \textbf{+0.24} {\scriptsize($\pm$ 0.05)}   \\
\midrule
\texttt{FedProx} &  72.78 & 76.51  & 82.61  & 91.24   &  54.40  &  75.23   &  89.06  & 94.89 \\
~~ \small{+ PGALRS}  &  \textbf{+0.41} {\scriptsize($\pm$ 0.16)} &  \textbf{+0.62} {\scriptsize($\pm$ 0.31)} & \textbf{+0.83} {\scriptsize($\pm$ 0.38)} &  \textbf{+0.11} {\scriptsize($\pm$ 0.01)}  & \textbf{+0.32} {\scriptsize($\pm$ 0.33)} & \textbf{+0.37} {\scriptsize($\pm$ 0.29)} &  \textbf{+0.56} {\scriptsize($\pm$ 0.15)} &  \textbf{+0.21} {\scriptsize($\pm$ 0.13)}  \\
% \midrule
\midrule
FedAvgM & 75.44 & 79.51  &  83.28 & 90.07   &  52.26 &  69.80  &  86.20 & 96.51 \\
~~ \small{+ PGALRS}  &  \textbf{+0.47} {\scriptsize($\pm$ 0.39)}  &  \textbf{+0.26} {\scriptsize($\pm$ 0.24)}&  \textbf{+3.40} {\scriptsize($\pm$ 1.29)} &   \textbf{+0.38} {\scriptsize($\pm$ 0.16)} &  \textbf{+2.90} {\scriptsize($\pm$ 1.46)}   &  \textbf{+0.56} {\scriptsize($\pm$ 0.43)} &  \textbf{+0.48} {\scriptsize($\pm$ 1.14)}   & \textbf{+0.58} {\scriptsize($\pm$ 0.34)}  \\
\midrule
FedAdam &  76.76  & 79.96 & 86.72 &  91.72 &   55.90  & 71.57  &  97.83 & 98.60 \\
~~ \small{+ PGALRS}  & -0.17 {\scriptsize($\pm$ 0.48)}  &  \textbf{+0.17} {\scriptsize($\pm$ 0.08)} &  \textbf{+1.75} {\scriptsize($\pm$ 1.39)} & \textbf{+0.09} {\scriptsize($\pm$ 0.02)}  & \textbf{+1.16} {\scriptsize($\pm$ 2.81)}   &  \textbf{+0.98} {\scriptsize($\pm$ 0.84)} &  \textbf{+0.15} {\scriptsize($\pm$ 0.20)}   & \textbf{+0.04} {\scriptsize($\pm$ 0.03)} \\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/various_sampling_strategies.tex <==
\begin{table}[t]
\caption{The results of using different client sampling strategies.}
\label{tab: various sampling strategies}
\vskip 0.15in
\begin{center}
 \setlength{\tabcolsep}{6.0pt}
\begin{small}
%\begin{sc}
\begin{tabular}{llcc}
\toprule
\multirow{2.5}{*}{Dataset} & \multirow{2.5}{*}{Method} & \multicolumn{2}{c}{Sampling Strategy}  \\
\cmidrule(lr){3-4}
 & & MD & AdaFL  \\
\midrule
\multirow{4.5}{*}{CIFAR-10} & FedAvg & 41.44 & 39.85 \\
& ~~ \small{+ FedGLAD} & \textbf{42.20} & \textbf{41.39}  \\ 
\cmidrule{2-4}
 & FedAvgM & 51.77 & 52.76 \\
 & ~~ \small{+ FedGLAD} & \textbf{53.85} & \textbf{53.68} \\
 \cmidrule{1-4}
\multirow{4.5}{*}{20NewsGroups} & FedAvg & 73.36 & 72.14 \\
& ~~ \small{+ FedGLAD} & \textbf{74.04} & \textbf{72.92} \\ 
\cmidrule{2-4}
 & FedAvgM & 75.22 &  76.18 \\
 & ~~ \small{+ FedGLAD} & \textbf{75.60} & \textbf{76.40} \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
